DropPos: Pre-Training Vision Transformers by Reconstructing Dropped Positions

As it is empirically observed that Vision Transformers (ViTs) are quite insensitive to the order of input tokens, the need for an appropriate self-supervised pretext task that enhances the location awareness of ViTs is becoming evident. To address this, we present DropPos, a novel pretext task designed to reconstruct Dropped Positions. The formulation of DropPos is simple: we first drop a large random subset of positional embeddings and then the model classifies the actual position for each non-overlapping patch among all possible positions solely based on their visual appearance. To avoid trivial solutions, we increase the difficulty of this task by keeping only a subset of patches visible. Additionally, considering there may be different patches with similar visual appearances, we propose position smoothing and attentive reconstruction strategies to relax this classification problem, since it is not necessary to reconstruct their exact positions in these cases. Empirical evaluations of DropPos show strong capabilities. DropPos outperforms supervised pre-training and achieves competitive results compared with state-of-the-art self-supervised alternatives on a wide range of downstream benchmarks. This suggests that explicitly encouraging spatial reasoning abilities, as DropPos does, indeed contributes to the improved location awareness of ViTs. The code is publicly available at https://github.com/Haochen-Wang409/DropPos.

==> sections/1.intro.tex <==
\section{Introduction}\label{sec:intro}


Learning extensible visual representations without any human annotations, known as self-supervised learning (SSL), has become a key challenge in the field of computer vision~\cite{he2020momentum, chen2020simple, he2022masked, grill2020bootstrap, wu2018unsupervised, chen2023vlp, wen2023editorial, qiu2023pre} since it enables efficient transfer to various downstream benchmarks~\cite{russakovsky2015imagenet, lin2014microsoft, zhou2017scene}.
%
To achieve this goal, researchers carefully design visual pretext tasks to produce appropriate supervision using \textit{only} images~\cite{wu2018unsupervised, bao2022beit, doersch2015unsupervised, zhang2016colorful}.
%
Among popular approaches, contrastive learning (CL)~\cite{he2020momentum, grill2020bootstrap, chen2020simple, wu2018unsupervised} and masked image modeling (MIM)~\cite{bao2022beit, wang2023hard, he2022masked, wei2022masked, xie2022simmim, liu2022exploring} have shown competitive performance.
%
% However, CL methods heavily rely on carefully-designed augmentations~\cite{chen2020simple, chen2020improved, caron2020unsupervised, caron2021emerging}, while MIM alternatives depend on pre-defined mask strategies~\cite{wang2023hard, xie2022simmim, bao2022beit} and suitable learning targets~\cite{wei2022masked}.
%
Despite the success of these methods, it is unclear whether they have fully exploited the representation learning capabilities of Vision Transformers (ViTs)~\cite{dosovitskiy2021image}.
%
Recently, researchers have shown that ViTs are relatively \textit{insensitive} to the order of input tokens~\cite{naseer2021intriguing, chen2021empirical, zhai2022position}, leading to the hypothesis that their promising scaling behavior is mainly due to their ability to model the relationship between \textit{unordered} input tokens.
%
This inspires us to explore a novel self-supervised pretext task that enhances the location awareness of ViTs as well as requires minimal prior knowledge.
%
This task is supposed to specifically focus on boosting the capacity to capture spatial features, particularly positional information.
%
% Specifically, we propose to boost the ability of ViTs to capture spatial features, particularly positional information, and enhance spatial understanding and reasoning abilities compared to previous methods by \textit{designing a brand-new pretext task}.


(i) discrepancy between pre-training and fine-tuning, (ii) trivial solutions, (iii) when to reconstruct the exact positions.


% Intuitively, solving jigsaw puzzles~\cite{noroozi2016unsupervised} requires the assembly of different pieces, and these puzzle pieces can produce a complete picture after being assembled.
%
% To this end, solving jigsaw puzzles naturally becomes a \textit{simple} pretext task, removing the need for both complex data augmentation techniques and reconstructing dense patch values.
%
To better understand how ViTs preserve positional information of image patches, we first revisit the standard forward procedure of ViTs.
%
Specifically, a sequence of positional embeddings (PEs)~\cite{vaswani2017attention} is added to patch embeddings.
%
Intuitively, by simply \textit{discarding} these PEs and reconstructing the position for each patch solely based on visual appearance, the model \textit{implicitly} learns the spatial arrangement.
%
However, this paradigm may lead to discrepancies between pre-training and fine-tuning, as the model has never been exposed to any PEs during pre-training.
%
To address this issue, we propose a simple and straightforward dropping strategy that urges ViTs to reconstruct \textit{dropped} positions (\method).
%
To be specific, \method randomly drops a \textit{large} portion of positional embeddings during pre-training and then prompts the model to \textit{classify the actual position} for each non-overlapping patch among all possible positions using a simple patch-wise classification objective.
%
\cref{fig-comparison} illustrates the benefits of \method, including (i) requiring less prior knowledge compared to CL, and (ii) not requesting a careful choice of target representation and mask strategy as MIM does.



Interestingly, we empirically find that ViTs perform extremely well on this position reconstruction task.
%
Therefore, to increase the difficulty of the task and avoid trivial solutions, we only keep a \textit{subset} of patches visible during pre-training.
%
For these visible patches, we randomly drop their positional embeddings, and the model is then required to reconstruct their positions based on the small subset of visual appearance and only a few anchors (\textit{i.e.}, patches with unmasked PEs).
%
To prevent the model from being overwhelmed by this particular task, we further introduce a position-smoothing strategy when predictions are close to the actual position.
%
Furthermore, to help the model focus on reconstructing the positions of salient areas, we propose an attentive reconstruction technique.
%
These two components are adopted when classifying the \textit{exact} positions of some particular patches are \textit{not} necessary.
%
Overall, \method offers a more streamlined approach to self-supervised learning as well as contributes to improved spatial understanding and reasoning abilities.


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/comparison.pdf}
    \vspace{-15pt}
    \caption{
    \textbf{Comparison between different pretext tasks.}
    %
    \textbf{(a)} Contrastive learning aims to maximize the agreement between different views of the same image.
    %
    \textbf{(b)} Masked image modeling predicts specific contents of masked patches.
    %
    \textbf{(c)} Our \method tries to reconstruct absolute positions based on only visual appearance.
    %
    \gc{Gray patches} on the \textit{top} of (b) and (c) do not contribute to training.
    %
    \gc{Gray patches} on the \textit{bottom} of (b) and (c) are \texttt{[MASK]} tokens.
    %
    % \method is a new simple and effective self-supervised pretext task and does not rely on augmentations and reconstructing specific patch values.
    }
    \label{fig-comparison}
    \vspace{-10pt}
\end{figure}


Through extensive experiments, we demonstrate that \method achieves competitive results compared with state-of-the-art alternatives on various downstream tasks.
%
Specifically, with only 800 epochs pre-training, \method achieves 84.2\% top-1 accuracy on ImageNet-1K~\cite{russakovsky2015imagenet} validation set using ViT-B/16~\cite{dosovitskiy2021image}, outperforming MAE~\cite{he2022masked} pre-trained with 1600 epochs by +0.6\%.
%
Moreover, on COCO~\cite{lin2014microsoft} object detection and ADE20k~\cite{zhou2017scene} semantic segmentation benchmarks, where these tasks require more abilities of spatial reasoning and understanding, \method achieves xx.x\% AP$^{\text{b}}$ fine-tuned with 1$\times$ schedule and xx.x\% mIoU fine-tuned with 80k iterations, outperforming MAE~\cite{he2022masked} under the exact same setting by +x.x\% and +x.x\%, respectively.



